Look Twice Before You Answer: Memory-Space Visual Retracing for Hallucination Mitigation in Multimodal Large Language Models

Despite their impressive capabilities, multimodal large language models (MLLMs) are prone to hallucinations, i.e., the generated content that is nonsensical or unfaithful to input sources. Unlike in LLMs, hallucinations in MLLMs often stem from the sensitivity of text decoder to visual tokens, leading to a phenomenon akin to "amnesia" about visual information. To address this issue, we propose MemVR, a novel decoding paradigm inspired by common cognition: when the memory of an image seen the moment before is forgotten, people will look at it again for factual answers. Following this principle, we treat visual tokens as supplementary evidence, re-injecting them into the MLLM through Feed Forward Network (FFN) as "key-value memory" at the middle trigger layer. This "look-twice" mechanism occurs when the model exhibits high uncertainty during inference, effectively enhancing factual alignment. Comprehensive experimental evaluations demonstrate that MemVR significantly mitigates hallucination across various MLLMs and excels in general benchmarks without incurring additional time overhead. The implementation is available from https://github.com/1zhou-Wang/MemVR

==> Tables/res_mask_experiment.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{1.0 \linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}[-0.5ex]{\textbf{Category}} & \multirow{2}{*}[-0.5ex]{\textbf{Type}} & \multicolumn{5}{c}{\textbf{Noise Step}} \\
\cmidrule(lr){3-7}					
 & & \textbf{500} & \textbf{600} & \textbf{700} & \textbf{800} & \textbf{900} \\
\midrule
\multirow{2}{*}{Perception} 
& Default & \textbf{1430.91} & 1338.85 & 1216.42 & 1061.55 & 897.39 \\
& Retraced & 1426.01 \downbad{4.90} & \textbf{1367.14} \up{28.29} & \textbf{1231.90} \up{15.48} & \textbf{1074.26} \up{12.71} & \textbf{899.64} \up{2.25} \\
\midrule
\multirow{2}{*}{Cognition} 
& Default & 302.00 & \textbf{307.14} & \textbf{296.07} & 280.71 & 318.57 \\
& Retraced & \textbf{312.50} \up{10.50} & 307.50 \up{0.36} & 294.64 \downbad{1.43} & \textbf{306.43} \up{25.72} & \textbf{328.93} \up{10.36} \\
\midrule
\multirow{2}{*}{Total (P+C)} 
& Default & 1732.91 & 1646.00 & 1512.49 & 1342.26 & 1215.97 \\
& Retraced & \textbf{1738.51} \up{5.60} & \textbf{1674.64} \up{28.64} & \textbf{1526.54} \up{14.05} & \textbf{1380.69} \up{38.43} & \textbf{1228.57} \up{12.60} \\
\bottomrule
\end{tabular}}
\vspace{1pt}
\caption{\textcolor{blue} {Noise experiment results of llava-v1.5-7b on MME, with Perception, Cognition, and Total (Per+Cog) at different noise steps. Best-performing method is highlighted in bold; arrows indicate improvement or degradation over the baseline, where higher values indicate better performance.}}
\label{tab:perception_cognition}
\end{table*}


==> Tables/res_selectlayer.tex <==
\begin{table*}[t!]\label{tab:res_layers}
\centering
\caption{Results of \modelname-static and \modelname-dynamic on MME. Static-\# indicates fixation on layer \# for visual retracing. \modelname-dynamic achieves optimal performance improvements.}
\vspace{-0.25em}
\resizebox{1.0 \linewidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
{Strategy} & Static-3\; & Static-7\; & Static-11 & Static-15 & Static-19 & Static-23 & Static-27 & Static-31 &  Dynamic  \\
\midrule
 Cognition & 364.64 & 347.14 & 362.86 & 352.14 & 350.36 & 357.86 & 355.71 & 346.43 &\bf 383.92 \\ 
 {Perception} & 1508.08 & 1500.48 & 1526.40 & \bf1529.07 & 1513.96 & 1500.29 & 1510.47 & 1510.34 & 1512.80 \\ \midrule
{Total Score} & 1872.72 & 1847.62 & 1889.26 & 1881.22 & 1864.32 & 1858.15 & 1866.18 & 1856.77 &\bf 1896.72 \\
\bottomrule
\end{tabular}}
\end{table*}
